CAGE: Causality-Aware Shapley Value for Global Explanations

As Artificial Intelligence (AI) is having more influence on our everyday lives, it becomes important that AI-based decisions are transparent and explainable. As a consequence, the field of eXplainable AI (or XAI) has become popular in recent years. One way to explain AI models is to elucidate the predictive importance of the input features for the AI model in general, also referred to as global explanations. Inspired by cooperative game theory, Shapley values offer a convenient way for quantifying the feature importance as explanations. However many methods based on Shapley values are built on the assumption of feature independence and often overlook causal relations of the features which could impact their importance for the ML model. Inspired by studies of explanations at the local level, we propose CAGE (Causally-Aware Shapley Values for Global Explanations). In particular, we introduce a novel sampling procedure for out-coalition features that respects the causal relations of the input features. We derive a practical approach that incorporates causal knowledge into global explanation and offers the possibility to interpret the predictive feature importance considering their causal relation. We evaluate our method on synthetic data and real-world data. The explanations from our approach suggest that they are not only more intuitive but also more faithful compared to previous global explanation methods.

==> backup/intro.tex <==
Artificial Intelligence (AI) systems have interwoven themselves into the societal framework, becoming indispensable in a myriad of applications ranging from creative endeavors such as recipe creation to critical decision-making processes in finance and criminal justice. The omnipresence of AI, exemplified by innovations like \textit{ChatGPT} and \textit{Bard}, has democratized technology, making it accessible beyond the tech-savvy circles to a broader spectrum of society. Whereas these examples are rather innocent, AI systems are also used to make life-changing decisions like loan accommodations \citep{sheikh2020approach} or if a person is released on parole \citep{berk2012criminal}. However, this pervasive influence underscores the urgent necessity for these systems to be transparent and explainable.

Explainable AI (XAI) has burgeoned as a field aiming to unveil the often obfuscated workings of AI models, fostering a deeper understanding and trust. However, the concept of ‘explanation’ within XAI is multifaceted, often bridging interpretability—the elucidation of a model’s architecture, with explanation—providing explicit, human-understandable reasons behind model decisions \cite{miller2019explanation}. Mittelstadt et al. \citep{mittelstadt2019explaining} and Miller \citep{miller2019explanation} consider explanations from a philosophical point of view and check if they correspond to the explanations in XAI. According to them, explanations are closely linked to causality. Humans give explanations of events and mechanisms with the help of counterfactuals. This means that they set up alternative realities and then estimate how that would change the outcome \citep{hume2000enquiry}.


%AI systems are already at the heart of society and are increasingly impacting our lives significantly. At the latest with the advent of chatbots like \textit{ChatGPT} (\url{https://openai.com/chatgpt}) or \textit{Bard} (\url{https://bard.google.com/}), it is no longer the tech-savvy milieu that uses these systems, but also other social groups are trying to take advantage of the possibilities of these language models. For instance, chefs let themselves create new recipes or copywriters trying to get inspiration or new ideas for their work. Whereas these examples are rather innocent, AI systems are also used to decide life-changing decisions like loan accommodations \citep{sheikh2020approach} or if a person is released on parole \citep{berk2012criminal}. Therefore, it is crucial that AI systems are explainable, fair, and well-understood. But worryingly this is not the case for the increasingly large and complex AI models.

%In order to remedy this situation, there have been a number of research projects in the last few years that have worked out possibilities for this in the field of explainable AI (XAI). The term explainable AI is not a unified scientific direction because there are different understandings of the term explanation. Miller \citep{miller2019explanation} works out two philosophies that complement each other in the field of XAI. One is \textit{interpretation}, which is more concerned with explaining decisions of a model in the context of its architecture. The other is \textit{explanation}, which is more focused on giving explicit explanations of model decisions for humans. So, in order for all people to be able to understand AI systems, work with them, and to be able to talk about them, one must first define what an explanation is in the first place. Mittelstadt et al. \citep{mittelstadt2019explaining} and Miller \citep{miller2019explanation} consider explanations from a philosophical point of view and check if it corresponds to the explanations in XAI. According to them, explanations are closely linked to causality. Humans give explanations of events and mechanisms with the help of counterfactuals. This means that they set up alternative realities and then estimate how that would change the outcome \citep{hume2000enquiry}.

Because explainable AI is not precisely defined, there are many approaches to explain artificial intelligence systems. One branch of research that has received a lot of attention and has also produced promising results is that of Shapley value-based methods. Two well-known frameworks are \textit{SHAP} \citep{lundberg2017unified} and \textit{SAGE} \citep{covert2020understanding}. Lloyd Shapley introduced \textit{Shapley values} in game theory \citep{shapley1953value}. They can be used to calculate the importance of individual players in a cooperative game, i.e., how much a player contributes to the outcome of a game. Roughly, the calculation is done by adding one player at a time to an existing subset of players and then calculating the increase in profit. This concept was translated into an XAI problem, among others, by Lundberg and Lee \citep{lundberg2017unified}. The problem with the translation is that ML models are inflexible and only work with a fixed number of features. It is not possible to just remove features and only provide a feature subset to the model. Therefore a way to let the model accommodate the features that are not provided in the subset, the missing features, needs to be found. In \textit{SHAP} and \textit{SAGE}, features are assumed to be independent. This allows a simple sampling procedure to be applied. Causal relations and dependencies between features are ignored. This has been pointed out by researchers to lead to incorrect and inaccurate explanations \citep{aas2021explaining, heskes2020causal, janzing2020feature, kumar2020problems}.


So, do \textit{Shapley value}-based explanation methods like \textit{SHAP} \citep{lundberg2017unified} and \textit{SAGE} \citep{covert2020understanding} correspond to the principles and definition of an explanation? Miller \citep{miller2019explanation} argues that humans arrive at their explanations through counterfactuals. Therefore, Kumar et al. \citep{kumar2020problems} tried to define \textit{Shapley values} as counterfactual statements, to match it with the cognitive approach of humans. But this approach remains constructed and not convincing. Also by the independence assumption, a causal component for an explanation is lost. This makes it clear that methods like \textit{SHAP} \citep{lundberg2017unified} and \textit{SAGE} \citep{covert2020understanding} in their original form have two weak points: The first one is more related to the philosophy of explanations \citep{miller2019explanation}. Since these methods are not oriented to how people arrive at explanations, they are difficult to apply for general explanations in a legal or social context. The second one is regarding the technical and mathematical problems of feature independence assumption. Research has shown that through this assumption methods like \textit{SHAP} and \textit{SAGE} become weaker explanation methods because they are vulnerable to adversarial attacks \citep{slack2020fooling} or assign misleading importance to features \citep{kumar2020problems, aas2021explaining}.

%\textit{SHAP} was extended in several studies to include a causal component in which the causal relationship between the features was taken into account \citep{heskes2020causal, aas2021explaining, janzing2020feature, jung2022measuring}. The results showed that the local explanations were more conclusive. But there is yet missing a framework to incorporate causality into a global explanation framework like \textit{SAGE}.

In this work, we argue that by incorporating causal concepts we can improve both of the above-mentioned weak points. We show this by incorporating causality into the global explanatory framework \textit{SAGE}. We hypothesize that by this we on the one hand get more coherent explanations that actually capture the true contributions of each feature and on the other hand that our causal method has closer links with the philosophy of explanations. These hypotheses are investigated by first performing experiments on synthetic data where the true importance of the features is known. Synthetic data is well suited to investigate the basic mechanisms of a method and to give a distinction and judgment whether the classical \textit{SAGE} method or the causal method gives better explanations. Furthermore, we will try our causal method on a real-world data application to investigate whether it is also applicable in this setting and delivers the desired results.

Accordingly, this work will make the following contributions:
\begin{enumerate}
    \item We expose shortcomings and inaccuracies in the hitherto widely used global explanation method \textit{SAGE}.
    \item We propose a global causal XAI method that incorporates causal knowledge.
    \item We argue that causality must become a necessary component of explainable artificial intelligence to be truly embraced by the broader society.
\end{enumerate}

%This paper is structured as follows: in the next Section, we will introduce explainable AI methods in a broader sense and explain related work that will be relevant to this paper. In Section 3 we will introduce terminology and concepts that we will use for our method. The causal method itself will be defined in Section 4. In Section 5 we will analyze the method with experiments and show and discuss the results. In the last Section, we will recap our findings and will evaluate them critically based on our hypothesis.









%%%%%%%%%%%%%%%%%%%%
\section{Related WOrk}
Explainable Artificial Intelligence (XAI) encompasses a vast domain where the essence of ‘explainability’ proves to be elusive and multifaceted, mirroring itself through a plethora of evolving approaches and methodologies. This section provides some relevant works through methods that conspicuously align with the thematic realms of this research.

A quintessential division within the realm of explanations bifurcates them into local and global variants. Local explanations gravitate towards elucidating individual predictions, encapsulating the essence of specific data instances, and unraveling the distinctive importance attributed to features for an individual instance \citep{bach2015pixel, ribeiro2016should, lundberg2017unified}. In contrast, global explanations pivot towards explaining the entire model mechanism by, for instance, providing the most important features for the model to make a prediction. For an extensive overview of different explainable AI methods, we refer to \citep{samek2021explaining}.

%As indicated in the Introduction, the field of explainable artificial intelligence itself is vast, and explainability as a concept is difficult to explain. This is also reflected in the many different emerging approaches to explainable AI. In this Section, we give an introduction to the methods that are relevant to this work. 

%On a superficial level, a distinction can be made between local and global explanations. The former tries to explain individual predictions of a model, i.e. explaining a particular instance of the input data and reason about the importance of the features on a specific instance \citep{bach2015pixel, ribeiro2016should, lundberg2017unified}. Approaches of the latter, on the other hand, are rather interested in the concepts and representations the model uses to make its prediction. On the basis of these explanatory objectives, many practical methods have been built to achieve these explanations. For an extensive overview of different explainable AI methods, we refer to \citep{samek2021explaining}.

The focus of this article is on methods that are based on \textit{Shapley values} \cite{shapley1953value}. The framework of \textit{Shapley values} originated in the context of game theory to measure the contribution of a player in a cooperative game \citep{shapley1953value}. Lundberg and Lee \citep{lundberg2017unified} picked up this idea of \textit{Shapley values} and translated it to an explainable AI problem to introduce their framework \textit{SHAP} which belongs to the class of additive feature attribution methods. This class combines different methods for local explanations. Translated to an explainable AI problem, \textit{Shapley values} do not measure a player's value in a cooperative game but rather to what extent a feature contributes to the output of a model.  

Since its inception, SHAP has evolved, adapting to a diverse array of tasks and explanatory objectives through various extensions and modifications. Notable among these are\textit{KernelSHAP} \citep{lundberg2017unified, covert2021improving}, \textit{TreeSHAP} \citep{lundberg2020local}, and \textit{LossSHAP} \citep{lundberg2020local, covert2020feature}. KernelSHAP, a model-agnostic explainable method, is appreciated for its adaptability across numerous model types. In contrast, TreeSHAP is specially tailored for tree models, offering dedicated insights into tree-based model interpretations. LossSHAP diverges in its explanatory focus. Rather than adhering to traditional approaches, it emphasizes the influence of features based on evaluation metrics. For instance, it evaluates the importance of a feature by analyzing its impact on specific evaluation criteria such as the mean squared error in regression contexts. 

The idea of \textit{Shapley values} has also been used to build global explanation methods. One method that is connected to \textit{SHAP} is that of Covert et al. (2020) where the authors develop a \textit{Shapley value}-based method for global feature importance called \textit{SAGE} \citep{covert2020understanding}. They also introduce additive importance measures as a similar class of methods like additive feature attribution methods \citep{lundberg2017unified}. In this class, the importance of a feature is defined as the predictive power that it contributes rather than the absolute effect it has on the prediction. This means that \textit{SAGE} measures if a feature makes a prediction more or less correct, according to evaluation metrics whereas \textit{SHAP}-based methods measure the pure change that features have on the prediction. \textit{SAGE} is, therefore, the global equivalent of \textit{LossSHAP}.

As discussed, all of these methods have issues and problems that can significantly distort or give misleading explanations. These issues can be attributed to the assumption that features are independent and that relations between features are ignored \citep{kumar2020problems, aas2021explaining, hooker2021unrestricted}. There have been several papers that investigate these shortcomings. Aas et al.  \citep{aas2021explaining} extend the \textit{KernelSHAP} method so that it can handle highly correlated features. Another line of studies investigates how feature dependencies and \textit{Shapley values} can be interpreted from a causal perspective. Frye et al. \citep{frye2020asymmetric} present \textit{Asymmetric Shapley values} where they incorporate causal knowledge by only allowing possible permutations of features that comply with the causal structure of the input features when computing \textit{Shapley values}. Janzing et al. \citep{janzing2020feature} tackle the question of how to deal with missing features in \textit{SHAP}-based methods. They replace conditional sampling in the \textit{Shapley value} computation with conditioning by intervention with do-calculus, a causal concept that was introduced by Judea Pearl \citep{pearl1995causal}. Similarly, Heskes et al. \citep{heskes2020causal} and Jung et al. \citep{jung2022measuring} use do-calculus to compute the causal contribution of a feature to the models' prediction. 

%By incorporating the causal knowledge about features into the explanation the authors demonstrate two things: (1) causal explanations are closer to the cognitive understanding of explanations in the sense that people understand explanations as a causal construct between cause and effect. (2) Through the causal intervention the often wrongful independence assumption of features can be neglected.
